Shadow Imaging of Transiting Objects

We consider the problem of inferring the shape of a transiting object's silhouette from its light curve alone, without assuming a physical model for the object. We model the object as a grid of pixels which transits the star; each pixel has an opacity, ranging from transparent to opaque, which we infer from the light curve. We explore three interesting degeneracies inherent to this problem, in which markedly different transiting shapes can produce identical light curves: (i) the "flip" degeneracy, by which two pixels transiting at the same impact parameter on opposite sides of the star's horizontal midplane generate the same light curve; (ii) the "arc" degeneracy, by which opacity can be redistributed along the semicircular arc of pixels which undergoes ingress or egress at the same time without consequence to the light curve, and (iii) the "stretch" degeneracy, by which a wide shape moving fast can produce the same light curve as a narrow shape moving more slowly. By understanding these degeneracies and adopting some additional assumptions, we are able to numerically recover informative shadow images of transiting objects, and we explore a number of different algorithmic approaches to this problem. We apply our methods to real data, including the TRAPPIST-1c,e,f triple transit and two dips of Boyajian's Star. We provide Python code to calculate the transit light curve of any grid and, conversely, infer the image grid which generates any light curve in a software package accompanying this paper, EightBitTransit.

==> journals.tex <==
%\newcommand{\aj}{{\it AJ}}%
          % Astronomical Journal
\newcommand{\actaa}{{\it Acta Astron.}}%
          % Acta Astronomica
%\newcommand{\araa}{{\it ARA\&A}}%
          % Annual Review of Astron and Astrophys
%\newcommand{\apj}{{\it ApJ}}%
          % Astrophysical Journal
%\newcommand{\apjl}{{\it ApJ}}%
          % Astrophysical Journal, Letters
%\newcommand{\apjs}{{\it ApJS}}%
          % Astrophysical Journal, Supplement
%\newcommand{\ao}{{\it Appl.~Opt.}}%
          % Applied Optics
%\newcommand{\apss}{{\it Ap\&SS}}%
          % Astrophysics and Space Science
%\newcommand{\aap}{{\it A\&A}}%
          % Astronomy and Astrophysics
%\newcommand{\aapr}{{\it A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
%\newcommand{\aaps}{{\it A\&AS}}%
          % Astronomy and Astrophysics, Supplement
%\newcommand{\azh}{{\it AZh}}%
          % Astronomicheskii Zhurnal
%\newcommand{\baas}{{\it BAAS}}%
          % Bulletin of the AAS
\newcommand{\caa}{{\it Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{{\it Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
%\newcommand{\icarus}{{\it Icarus}}%
  % Icarus
\newcommand{\jcap}{{\it J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
%\newcommand{\jrasc}{{\it JRASC}}%
          % Journal of the RAS of Canada
%\newcommand{\memras}{{\it MmRAS}}%
          % Memoirs of the RAS
%\newcommand{\mnras}{{\it MNRAS}}%
          % Monthly Notices of the RAS
\newcommand{\na}{{\it New A}}%
  % New Astronomy
\newcommand{\nar}{{\it New A Rev.}}%
  % New Astronomy Review
%\newcommand{\pra}{{\it Phys.~Rev.~A}}%
          % Physical Review A: General Physics
%\newcommand{\prb}{{\it Phys.~Rev.~B}}%
          % Physical Review B: Solid State
%\newcommand{\prc}{{\it Phys.~Rev.~C}}%
          % Physical Review C
%\newcommand{\prd}{{\it Phys.~Rev.~D}}%
          % Physical Review D
%\newcommand{\pre}{{\it Phys.~Rev.~E}}%
          % Physical Review E
%\newcommand{\prl}{{\it Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand{\pasa}{{\it PASA}}%
  % Publications of the Astron. Soc. of Australia
%\newcommand{\pasp}{{\it PASP}}%
          % Publications of the ASP
%\newcommand{\pasj}{{\it PASJ}}%
          % Publications of the ASJ
%\newcommand{\qjras}{{\it QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand{\rmxaa}{{\it Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\skytel}{{\it S\&T}}%
          % Sky and Telescope
%\newcommand{\solphys}{{\it Sol.~Phys.}}%
          % Solar Physics
%\newcommand{\sovast}{{\it Soviet~Ast.}}%
          % Soviet Astronomy
%\newcommand{\ssr}{{\it Space~Sci.~Rev.}}%
          % Space Science Reviews
%\newcommand{\zap}{{\it ZAp}}%
          % Zeitschrift fuer Astrophysik
%\newcommand{\nat}{{\it Nature}}%
          % Nature
%\newcommand{\iaucirc}{{\it IAU~Circ.}}%
          % IAU Cirulars
%\newcommand{\aplett}{{\it Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
%\newcommand{\apspr}{{\it Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
%\newcommand{\bain}{{\it Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
%\newcommand{\fcp}{{\it Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
%\newcommand{\gca}{{\it Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
%\newcommand{\grl}{{\it Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
%\newcommand{\jcp}{{\it J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
%\newcommand{\jgr}{{\it J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
%\newcommand{\jqsrt}{{\it J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand{\memsai}{{\it Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%\newcommand{\nphysa}{{\it Nucl.~Phys.~A}}%
          % Nuclear Physics A
%\newcommand{\physrep}{{\it Phys.~Rep.}}%
          % Physics Reports
%\newcommand{\physscr}{{\it Phys.~Scr}}%
          % Physica Scripta
%\newcommand{\planss}{{\it Planet.~Space~Sci.}}%
          % Planetary Space Science
%\newcommand{\procspie}{{\it Proc.~SPIE}}%
          % Proceedings of the SPIE
